Equivariant Denoisers Cannot Copy Graphs: Align Your Graph Diffusion Models

Graph diffusion models, dominant in graph generative modeling, remain underexplored for graph-to-graph translation tasks like chemical reaction prediction. We demonstrate that standard permutation equivariant denoisers face fundamental limitations in these tasks due to their inability to break symmetries in noisy inputs. To address this, we propose aligning input and target graphs to break input symmetries while preserving permutation equivariance in non-matching graph portions. Using retrosynthesis (i.e., the task of predicting precursors for synthesis of a given target molecule) as our application domain, we show how alignment dramatically improves discrete diffusion model performance from 5% to a SOTA-matching 54.7% top-1 accuracy. Code is available at https://github.com/Aalto-QuML/DiffAlign.

==> figures/components.tex <==
\newcommand{\noisySample}{
    \draw circle (4pt);
    \draw (0.1, 0.6) circle (4pt);
    \draw (-0.3, 1.2) circle (4pt);
    \draw (-0.2, 0.85) circle (4pt);
    \draw (-1, 1) circle (4pt);
    \draw (-0.6, 0.9) circle (4pt);
    \draw (-0.95, 0.2) circle (4pt);
    \draw (-0.35, 0.5) circle (4pt);
    \draw (-0.75, 0.5) circle (4pt);
    \draw (-0.6, 0) circle (4pt);
    \draw (-0.3, 0.16) circle (4pt);
    \draw (0.4, 0.4) circle (4pt);
}

\newcommand{\conditioningProduct}[1][1]{
    \node at (-0.5*#1,1.2*1) {product};
    \node {\scalebox{#1}{\chemfig{*6(=-=(-CH_3)-(-[:90]\textcolor{red}{OH})-\textcolor{blue}{N}-=)}}};
}    

\newcommand{\SampleWithoutAMPE}[1][1]{ % Default scale factor is 1
    \node at (0.2 * #1, -1 * #1) {\scalebox{#1}{\textcolor{blue}{\chemfig{BH_3}}}};
    \node at (0, 0.5 * #1) {\scalebox{#1}{\chemfig{CH_4}}};
    \node at (-0.3 * #1, -0.4 * #1) {\scalebox{#1}{\chemfig{CH_4}}};
    \node at (1.3 * #1, -0.8 * #1) {\scalebox{#1}{\chemfig{CH_4}}};
    \node at (1.3 * #1, 0.2 * #1) {\scalebox{#1}{\chemfig{C=\textcolor{blue}{N}}}};
    \node at (0.7 * #1, -0.35 * #1) {\scalebox{#1}{\chemfig{NH_3}}};
}

\newcommand{\SampleWithAMPE}[1][1]{ % Default scale factor is 1
    \node {\scalebox{#1}{\chemfig[atom sep=2.2em]{*6(=-=(-CH_3)-(-[:90]\textcolor{red}{OH})-\textcolor{blue}{N}-=)}} };
    \node at (1.5 * #1, -1 * #1) { \scalebox{#1}{\chemfig{\textcolor{red}{H_2O}}} };
}

\newcommand{\ModelWithoutAMPE}{
    \node (labelWithout) at (-1,1.2) { \footnotesize $\mathbf{X}_0 \sim p_{\theta}(\mathbf{X}_0|\mathbf{X}_T, \mathbf{P})$};
}
\newcommand{\ModelWithAMPE}{
    \node (labelWith) at (3,1.2) {\footnotesize $\mathbf{X}_0 \sim p_{\theta}(\mathbf{X}_0|\big[\mathbf{X}_T, \mathbf{E}\big], \mathbf{P})$};
}

==> figures/fig-app-ampe-vs-noampe.tex <==
\input{figures/components}
\newcommand{\ampedXAxis}{1.7} 
\newcommand{\condLineXAxis}{15.5} 
\newcommand{\condProdXAxis}{17} 
\newcommand{\spaceBetweenSamplesHorizontal}{0.43} 
\newcommand{\sampleWidth}{2.5} 
\setchemfig{bond style={line width=1.2pt}}

\begin{tikzpicture}
    % Create the blocks
    \begin{scope}[shift=({\condProdXAxis,0})]% Adjust the shift values as needed
        \conditioningProduct[0.5]
    \end{scope}
    
    \draw (\condLineXAxis,2.8) -- (\condLineXAxis,-2.8);

    \node at (0,1.5) [align=center, text width=1cm] {With PE}; % Adjust position and text as needed
    \node at (0,-1.7) [align=center, text width=1cm] {Without PE}; 

    \node at (\ampedXAxis,3) {t=T};
    \begin{scope}[shift={(\ampedXAxis+\spaceBetweenSamplesHorizontal,1)}]
        \noisySample
    \end{scope}

    \node[scale=1] at (\ampedXAxis+\sampleWidth+\spaceBetweenSamplesHorizontal,3) {t=0};
    \begin{scope}[shift={(\ampedXAxis+\sampleWidth+\spaceBetweenSamplesHorizontal,1.5)}] % Adjust the shift values as needed
        \SampleWithAMPE[0.7] % Apply scaling
    \end{scope}

    \node[scale=1] at ($(\ampedXAxis,3) + (\sampleWidth*2+\spaceBetweenSamplesHorizontal*2,0)$) {t=0};
    \begin{scope}[shift={($(\ampedXAxis,1.5) + (\sampleWidth*2+\spaceBetweenSamplesHorizontal*2,0)$)}] % Adjust the shift values as needed
        \SampleWithAMPE[0.7] % Apply scaling
    \end{scope}

    \node[scale=1] at ($(\ampedXAxis,3) + (\sampleWidth*3+\spaceBetweenSamplesHorizontal*3,0)$) {t=0};
    \begin{scope}[shift={($(\ampedXAxis,1.5) + (\sampleWidth*3+\spaceBetweenSamplesHorizontal*3,0)$)}] % Adjust the shift values as needed
        \SampleWithAMPE[0.7] % Apply scaling
    \end{scope}

    \node[scale=1] at ($(\ampedXAxis,3) + (\sampleWidth*4+\spaceBetweenSamplesHorizontal*4,0)$) {t=0};
    \begin{scope}[shift={($(\ampedXAxis,1.5) + (\sampleWidth*4+\spaceBetweenSamplesHorizontal*4,0)$)}] % Adjust the shift values as needed
        \SampleWithAMPE[0.7] % Apply scaling
    \end{scope}

    \begin{scope}[shift={(\ampedXAxis+0.3,-2.3)}]
        \noisySample
    \end{scope}
    
    \begin{scope}[shift={(\ampedXAxis+\sampleWidth+\spaceBetweenSamplesHorizontal-0.7,-1.1)}] % Adjust the shift values as needed
        \SampleWithoutAMPE[0.7] % Apply scaling
    \end{scope}

    \begin{scope}[shift={($(\ampedXAxis,-1.5) + (\sampleWidth*2+\spaceBetweenSamplesHorizontal*2,0)$)}] % Adjust the shift values as needed
        \SampleWithoutAMPE[0.7] % Apply scaling
    \end{scope}

    \begin{scope}[shift={($(\ampedXAxis,-1.5) + (\sampleWidth*3+\spaceBetweenSamplesHorizontal*3,0)$)}] % Adjust the shift values as needed
        \SampleWithoutAMPE[0.7] % Apply scaling
    \end{scope}

    \begin{scope}[shift={($(\ampedXAxis,-1.5) + (\sampleWidth*4+\spaceBetweenSamplesHorizontal*4,0)$)}] % Adjust the shift values as needed
        \SampleWithoutAMPE[0.7] % Apply scaling
    \end{scope}
    
    % Additional details like arrows and labels can be added here
\end{tikzpicture}


==> figures/fig4-ampe-vs-noampe-legacy.tex <==
\begin{tikzpicture}
    % % Label for Noise Sample, positioned higher
    \node[anchor=south] at (0,4.3) {\footnotesize $\mathbf{X}_T \sim p(\mathbf{X}_T)$};

    % Top left portion (Noise Sample)
    \foreach \x in {-1.5,-0.5,...,1.5}
        \foreach \y in {2.5,3.0,...,3.5}
            \filldraw (\x, \y) circle (2pt); % Example nodes for noise sample

    % Vertical line separator
    \draw (2.4,2) -- (2.4,3.6);

    % Top right portion (Product Molecule)
    % Draw the product molecule to the right of the separator
    \node at (4.3,3) {\scalebox{\moleculeScale}{\chemfig{*6(=-=(-CH_3)-(-[:90]\textcolor{red}{OH})-\textcolor{blue}{N}-=)}}};

    \node[anchor=south] at (3.8,4.3) {\footnotesize $\mathbf{P}$};

    % Define the center point and adjusted radii
    \def\centerX{-1}
    \def\centerY{-1}
    \def\sideRadius{0.75} % Smaller radius for side fragments
    \def\upperLowerRadius{1.5} % Radius for upper and lower fragments

    % Manually place each molecule fragment
    \scalebox{\moleculeScale}{
        \node at (\centerX + \sideRadius, \centerY) {\textcolor{blue}{\chemfig{BH_3}}};
        \node at (\centerX + \upperLowerRadius*cos{60}, \centerY + \upperLowerRadius*sin{60}) {\chemfig{CH_4}};
        \node at (\centerX + \upperLowerRadius*cos{120}, \centerY + \upperLowerRadius*sin{120}) {\chemfig{CH_4}};
        \node at (\centerX, \centerY + \upperLowerRadius) {\chemfig{CH_4}};
        \node at (\centerX - \sideRadius, \centerY) {\chemfig{C=\textcolor{blue}{N}}};
        \node at (\centerX, \centerY - \upperLowerRadius) {\chemfig{NH_3}};
    }

    % Bottom Right (Denoiser with Positional Encodings)
    \node (denoiserWith) at (3,-0.5) {\scalebox{\moleculeScale}{ % Lower position
        \chemfig{*6(=-=(-CH_3)-(-[:90]\textcolor{red}{OH})-\textcolor{blue}{N}-=)} \quad \chemfig{\textcolor{red}{H_2O}}}
    };

    % \node (labelWithout) at (-4.5,1.2) {\small $\mathbf{X}_0 \sim p_{\theta}(\mathbf{X}_0|\mathbf{X}_T, \mathbf{P})$};
    % \node (labelWith) at (5.5,1.2) {\small $\mathbf{X}_T \sim p_{\theta,AMPED}(\mathbf{X}_0|\big[\mathbf{X}_T, \mathbf{E}\big], \mathbf{P})$};

    % \draw[-{Latex[length=3mm]}] (-1,2.5) -- (labelWithout);
    % \draw[-{Latex[length=3mm]}] (1,2.5) -- (labelWith);

    % Arrows from Noise Sample to the labels, with labels positioned near the arrows
    % \draw[-{Latex[length=3mm]}] (0,1.5) -- (-0.5,0.5) 
    %     node[midway, above, left] {\small $p_{\theta}(\mathbf{X}_0|\mathbf{X}_T, \mathbf{P})$};

    % \draw[-{Latex[length=3mm]}] ((1,1.5) -- (1.5,0.5) 
    %     node[midway, above, right] {\small $p_{\theta}(\mathbf{X}_0|\big[\mathbf{X}_T, \mathbf{E}\big], \mathbf{P})$};

    % Labels for denoised molecules, positioned below the arrow start points
    \node (labelWithout) at (-1,1.2) { \footnotesize $\mathbf{X}_0 \sim p_{\theta}(\mathbf{X}_0|\mathbf{X}_T, \mathbf{P})$};
    \node (labelWith) at (3,1.2) {\footnotesize $\mathbf{X}_0 \sim p_{\theta}(\mathbf{X}_0|\big[\mathbf{X}_T, \mathbf{E}\big], \mathbf{P})$};

    % Arrows from Noise Sample to the labels
    % \draw[-{Latex[length=3mm]}] (-1,2.5) -- (labelWithout);
    % \draw[-{Latex[length=3mm]}] (1,2.5) -- (labelWith);
\end{tikzpicture}


==> figures/fig4-ampe-vs-noampe.tex <==
\input{figures/components}
\newcommand{\ampedXAxis}{2.3} 
\newcommand{\condLineXAxis}{7.5} 
\newcommand{\condProdXAxis}{9} 

\begin{tikzpicture}
    % Create the blocks
    \begin{scope}[shift=({\condProdXAxis,0})]% Adjust the shift values as needed
        \conditioningProduct[0.5]
    \end{scope}
    
    \draw (\condLineXAxis,2.8) -- (\condLineXAxis,-2.8);

    \node at (0,1.5) [align=center, text width=1cm] {With PE}; % Adjust position and text as needed
    \node at (0,-1.7) [align=center, text width=1cm] {Without PE}; 
        
    % \draw (2.6,0.6) -- (2.6,2.7);
    % \draw (2.6,-0.7) -- (2.6,-2.8);
    
    \node at (\ampedXAxis,3) {$t=T$};
    \begin{scope}[shift={(\ampedXAxis+0.3,1)}]
        \noisySample
    \end{scope}

    \node[scale=1] at (\ampedXAxis+2.5,3) {$t=0$};
    \begin{scope}[shift={(\ampedXAxis+3,1.5)}] % Adjust the shift values as needed
        \SampleWithAMPE[0.7] % Apply scaling
    \end{scope}

    \begin{scope}[shift={(\ampedXAxis+0.3, -2.3)}]
        \noisySample
    \end{scope}
    
    \begin{scope}[shift={(\ampedXAxis+2.5,-1.5)}] % Adjust the shift values as needed
        \SampleWithoutAMPE[1] 
    \end{scope}
    
    % Additional details like arrows and labels can be added here
\end{tikzpicture}

